Adversarial Robustness Certification for Bayesian Neural Networks

We study the problem of certifying the robustness of Bayesian neural networks (BNNs) to adversarial input perturbations. Given a compact set of input points $T \subseteq \mathbb{R}^m$ and a set of output points $S \subseteq \mathbb{R}^n$, we define two notions of robustness for BNNs in an adversarial setting: probabilistic robustness and decision robustness. Probabilistic robustness is the probability that for all points in $T$ the output of a BNN sampled from the posterior is in $S$. On the other hand, decision robustness considers the optimal decision of a BNN and checks if for all points in $T$ the optimal decision of the BNN for a given loss function lies within the output set $S$. Although exact computation of these robustness properties is challenging due to the probabilistic and non-convex nature of BNNs, we present a unified computational framework for efficiently and formally bounding them. Our approach is based on weight interval sampling, integration, and bound propagation techniques, and can be applied to BNNs with a large number of parameters, and independently of the (approximate) inference method employed to train the BNN. We evaluate the effectiveness of our methods on various regression and classification tasks, including an industrial regression benchmark, MNIST, traffic sign recognition, and airborne collision avoidance, and demonstrate that our approach enables certification of robustness and uncertainty of BNN predictions.

==> Sections/Background_old.tex <==
\section{Background}




\subsection{Local Robustness}

Here, we formally define adversarial examples as violations of a \textit{local robustness property}. As with deterministic neural networks, we say that a sample from a BNN $f^{w}$ is \textit{robust} with respect to an input $x$ if there is no perturbation of $x$ within an allowed input set $T$ which causes the output of $f^{w}$ to be outside of $S$.
\ap{Imho, you have to introduce BNNs before introducing those definitations, otherwise the notation is all up in the air.}
\begin{restatable}[Local Robustness Property]{definition}{localpropertydet}\label{def:localpropertydet}
Given a sample from a BNN $f^{w}$ with weights fixed to $w$, an input $x$, an input set $T\subseteq \mathbb{R}^{n}$ including $x$, and a set $S\subseteq \mathbb{R}^{m}$ \ap{before it was m, nc, and now is n and m...} of safe outputs, we say the network is locally robust at $x$ if and only if
\begin{align}
    f^{w}(x') \in S \quad \forall x' \in T
\end{align}
\end{restatable}
We can then simply state the formal definition of an adversarial example as a violation of this local robustness property (equivalently, when local robustness is not satisfied): 
\begin{restatable}[Adversarial Example]{definition}{adversarialexample}\label{def:adversarialexample}
Given a sample from a BNN $f^{w}$ with weights fixed to $w$, an input $x$, an input set $T\subseteq \mathbb{R}^{n}$ such that $x \in T$, and a set $S\subseteq \mathbb{R}^{m}$ of safe outputs, we say that an input $x'$ is an adversarial example iff:
\begin{align}
    \*x' \in T \quad \wedge \quad f^{\theta}(\*x') \notin S  
\end{align}
\ap{theta?}
\end{restatable}
If a network satisfies the conditions of Definition~\ref{def:localpropertydet} we say it is \textit{robust} \ap{This is very confusing, because all of these statements are for the deterministic version. A reviewer will not understand this, unless you tell them that something else will come later...}. Conversely, if an input satisfies Definition~\ref{def:adversarialexample} then we say it is \textit{vulnerable} or \textit{non-robust}.

\paragraph{Input Specifications}

The choice of input set $T$ depends entirely on the application and desired specification. For industrial applications $T$ may encompass all points that are within worst-case instrumental noise. For images, we may try to capture all semantically identical images in $T$ \ap{This is wrong I think. All semantically identical images of a horse for example, include also horses which are very different from a horse. To identify all the semantically identical images of something is not the task of verification, it's the task of learning}. As we deal with local properties the one thing each set $T$ will have is the inclusion of $x$. images, Despite the lack of a one-size-fits-all input specification, it is often the case that an $\ell_p$-norm ball is a general and interesting specification for most domains. We recall the definition of an $\ell_p$-norm ball centered at $x$ here:  \ap{You do not need to define formally what an ellp ball is. Everyone know what it is. and if you really want to define it, you can just give it inline....}
\begin{definition}\label{def:ellpball}
Given a vector $\*x \in \mathbb{R}^{in}$ the $\ell_p$ norm ball of radius $\epsilon$ around $\*x$ is defined as:
\begin{align}
    \mathcal{B}_{\epsilon, p}(\*x) := \{ \*x' \ s.t. \ ||\*x' - \*x ||_p \leq \epsilon \}
\end{align}
\end{definition}
\ap{You can't have so much space talking about soemthing as trivial as a p-norm ball, imho, it's a bit pedantic}
One can select parameters of the norm ball ($\epsilon$ and $p$) in order to fine-tune the input property to the domain. While this ball does not typically capture \textit{all} of the semantically similar inputs for images, it can be tuned to capture a subset or superset of them. The $\ell_p$-norm ball setting is able to express different specifications with different settings of $p$, namely $p \in \{0, 1, 2, \infty \}$. For $p=0$, we recover the Hamming distance, which is simply a count of the number of dimensions which differ between $\*x'$ and $\*x$. For $p=1$, we recover the `Manhattan' distance which is simply the distance one would have to walk between $\*x'$ and $\*x$ if you were following a strict grid (as in a city blocks, hence Manhattan) in each dimension. For $p=2$ we have the straight-line or Euclidean distance. Finally, the $p=\infty$ is the most widely used metric. Also known as the sup norm, by definition, the $\ell_\infty$ norm measures the maximum difference between any two dimensions of the inputs. %In other words, $|| \*x - \*x' ||_\infty = max_{i \in [n]} |\*x_i - \*x'_i |$ given that $\*x \in \mathbb{R}^{in}$.
We note that the selection of $\epsilon$ ought to depend greatly on the selection of $p$. For instance, if one chooses $\ell_0$ then the value of $\epsilon$ will be an integer between 1 and $n$. For $\ell_\infty$, on the other hand, we would expect it to be in the interval $[0, 1]$ if the dimensions are normalized into that range. Further works, generally in fairness (which has strong links to robustness \cite{nanda2021fairness}), investigates ``balls'' of input points within a certain Mahalanobis distance of one another which allows the modeller to account for intracorrelation between input features  \cite{yurochkin2019training}. 

\paragraph{Output Specifications}

%It is clear that, if a traffic light is red and is predicted to be green (due perhaps to some noise in $\mathcal{B}_{1/255, \infty}$), we would say that prediction is unsafe. However, in general, it is difficult to determine what kind of change in prediction is \textit{unsafe}. 
Similarly to the input specifications there are some general measures which are typically of at least some interest to each application. For classification, generally one checks if there is an $x' \in T$ which causes the classification to change. This would be modelled as $S$ being all softmax vectors such that the true class maximal \ap{Something is missing from this sentence}. One could similarly check if there is an $\*x' \in T$ which causes the network to output a particular, unsafe class. This would be modelled as $S$ being all of the softmax vectors such that all but the particular unsafe class is maximal. For regression tasks, there is often some minor tolerated noise in the output and this is typically expected to be bounded w.r.t. the $\ell_2$ magnitude. One typical specification of interest is the Lipschitz property of a neural network. Formally, a network is Lipschitz continuous or $k$-Lipschitz continuous if it satisfies the following property for all $\*x^{(1)}, \*x^{(2)}$: $||f^{w}(\*x^{(1)}) - f^{w}(\*x^{(2)})||_p < k ||\*x^{(1)} - \*x^{(2)}||_p$. We note that in the case of using $\mathcal{B}_{\epsilon, p}$ as well as an $\ell_q$ norm in the output space, one is effectively providing a Lipschitz constraint on the function learned by the neural network.  \ap{This is wrong. I don't think the two problems are equivalent at all. Lipschitz continuity is way more restrictive. From adversarial robustness you cannot infere a Lipschitz constant. But from a Lipschitz constant you can over-approximated adversarial robsutness.}

No matter what the output specification is, we make the following assumption on $S$.
\begin{assumption}\label{assumption}
We assume that ${S}$ is described by $n_S$ linear constraints on the values of the final layer of the BNN, that is, 
$$ S=\{y\in \mathbb{R}^{n_c} \, |  \, C_S y + d_S \geq 0, C_S \in \mathbb{R}^{n_S\times n_c},d_S\in \mathbb{R}^{n_S}   \}  $$
\end{assumption}

We stress that, as discussed in \cite{gowal2018effectiveness}, this assumption encompasses most properties of interest for the verification of neural networks. We refer to $C_S y + d_S \geq 0$ as the \textit{safety specification} associated to the safe set $S$.
Below, in Example \ref{ex:Running}, we illustrate the notion of probabilistic safety on an example.

\subsection{Bayesian Neural Networks}

In this section we briefly review Bayesian neural networks and recall research which studies their robustness. We write $\BNN = [f_1^{\mathbf{w}}(x),\ldots,f_{n_c}^{\mathbf{w}}(x)]$ to denote a BNN with $n_c$ output units and an unspecified number of hidden layers, where ${\mathbf{w}}$ is the weight vector random variable.
The primary distinction between a BNN and a DNN is the distribution over ${\mathbf{w}}$ where $w \in \mathbb{R}^{n_w}$, a weight vector sampled from the distribution ${\mathbf{w}} \sim \post$. We denote with ${f}^w(x)$ the corresponding deterministic neural network with weights fixed to $w$.
In order to arrive at the final (posterior) distribution over weights one starts with a prior distribution i.e.\ $ {\mathbf{w}} \sim p(w)$, which one hopes captures all of the functions likely to fit the data. 
We focus soley on the supervised learning scenario in which we have access to a training set, $ \mathcal{D} =\{(x_i,y_i), i \in \{1,...,N_{\mathcal{D}} \} \}$. 
Learning amounts to computing the posterior distribution over the weights, $p (w \vert \mathcal{D} )$, via the application of Bayes rule. Given a posterior, we compute predictions, $y^*$, at an unseen input, $x^*$, via the posterior predictive distribution: 
\begin{align}\label{eq:posteriorpredictive}
    p(\*y^* | \*x^*, \mathcal{D}) = \int p(\*y^{*} | \*x^{*}, w)p(w | \mathcal{D}) dw
\end{align}
Unfortunately, because of the non-linearity introduced by the neural network architecture, the computation of the posterior and posterior predictive cannot be done analytically \cite{mackay1992practical}. In this work we derive specific procedures for the most commonly used posterior approximations, namely Gaussian Variational Inference (VI) approximations \cite{blundell2015weight} and Markov Chain Monte Carlo (MCMC) approximations. 

In particular, VI proceeds by finding a suitable Gaussian approximating distribution $q(w) = \mathcal{N}(w|\mu,\Sigma)$ for the posterior distribution, i.e.\ such that $ q(w) \approx p(w \vert \mathcal{D})$ \cite{oh1992vi}. 
The core idea is that the mean and covariance of  $q(w)$ are
iteratively optimized by minimizing a divergence measure between $q (w)$ and $ p (w | \mathcal{D})$.  The resulting approximate posterior takes the form $\mathcal{N}(w|\mu,\Sigma)$ where both $\mu$ and $\Sigma$ have been optimized \cite{oh1992vi, blundell2015weight, khan2018fast}.

Hamiltonian Monte Carlo (HMC) approximates the posterior by defining a Markov chain whose stationary distribution is $p(\theta | \mathcal{D})$ \cite{neal2012bayesian}. The primary advantage of such an approach is that in the limit of infinitely many samples, HMC will converge its stationary distribution, in this case, the true Bayesian posterior distribution.
HMC proceeds by exploring the Markov Chain using Hamiltonian dynamics to improve efficiency of the exploration. Unlike variational inference, the result of using an MCMC method such as HMC is a discrete number of samples which approximately represent the posterior, rather than a closed form distribution \cite{neal2012bayesian}.

In Section \ref{sec:methodology} we give explicit bounds for BNN certification for variational inference and Markov Chain Monte Carlo; however, we remark that the techniques developed in this paper  also extend to other classes of distributions and approximate inference methods, such as dropout  \cite{gal2016dropout}, with the caveat that in those cases the integral %for the safety computation 
in Eqn.\ \eqref{Eq:IntegralSafety}  (Section \ref{sec:methodology}) will not be Gaussian or discrete and will need to be computed by means of Monte Carlo sampling techniques.

==> Sections/Experiments_old.tex <==
\begin{figure*}
    \centering
    \subfigure{\includegraphics[width=0.48\textwidth]{Figures/MNIST.pdf}} 
    \subfigure{\includegraphics[width=0.48\textwidth]{Figures/FMNIST.pdf}}
    \caption{\textbf{Left:} Correctness analysis on MNIST. Over 1000 test set instances we plot the lower bound guarantee i.e. no adversary can force the true probability below the threshold. We find that for a large majority of inputs we can certify the decision up to $\epsilon = 0.075$. \textbf{Right:} Uncertainty analysis on FashionMNIST. Over 1000 test set instances we plot the maximum uncertain radius: we guarantee that no adversary can find a input within $\epsilon$ that causes the BNN to be certain. We find that for a large majority of the inputs we guarentee uncertainty up to $\epsilon=0.065$}
    \label{fig:MNISTAnalysis}
\end{figure*}

\section{Experiments}\label{sec:experiments}
In this section we use our framework for certification of Bayesian Neural Networks in order to perform a range of correctness analyses. 
\ap{Give sections references to where each of these things is happening.}
We start with an analysis of the Horizontal airborne Collision Avoidance System (HCAS) where we compute probabilistic safety bounds over the entire input space and analyse the tightness of our bounds on the posterior predictive mean. Next we study two industrial regression problems from the UCI dataset repository. We find that we can extend our bounds in order to compute the maximum safe radius and minimum unsafe radius for given properties. We study how our problem scales to medium sized inputs with the MNIST hand-written digit dataset where we are able to get tight bounds for networks with hundreds of thousands of weights. We also find that we are able to certify the network correctly produces uncertain behavior on out-of-distribution inputs. Finally, we study the German Traffic Sign Recognition Benchmark (GSTRB) in order to show how our method can efficently certify convolutional neural networks on inputs with thousands (2,352) of input dimensions.

We describe training methodology in each respective section and leave hyperparameters to the Appendix.


\subsection{Airborne Collision Avoidance}
%\ap{In my opinion we need a prove of correctes of the bound itself. Say for example estimating the results using IJCAI and showing that our bounds lie beneath it.}
We start our empirical investigation with the Horizontal airborne Collision Avoidance System (HCAS) \cite{julian2019guaranteeing}. The task of the neural networks in the HCAS problem is to take as input the information about the geometric layout (heading, location, and speed) of the ownship and an intruder, and return a warning if the ownship's current heading puts it on course for a near midair collision (NMAC). The HCAS dataset consists of roughly 20 million examples of intruder scenarios, each of which is described using four variables, displayed in the top right component of Figure~\ref{fig:HCASAnalysis}. There are four input variables describing the scenario and five possible advisories corresponding to five output dimensions, these are described in the top left portion of Figure~\ref{fig:HCASAnalysis}. Each output is assigned a real-valued \textit{reward}. The maximum reward advisory indicates the safest warning given the current intruder geometry. The advisories indicate the action a pilot should take to avoid a NMAC. These include clear of conflict (COC) advising no action, weak left (WL) advising a 2\textdegree/s left turn, weak right (WR) advising a 2\textdegree/s right turn, strong left (SL) advising a 4\textdegree/s left turn, and strong right (SR) advising a 4\textdegree/s right turn. Scenarios are then broken up based on time-to-collision and previous advisory. For each pair time-to-collision and previous advisory, we train a BNN to produce the correct current advisory, as is done with NNs in the original system in \cite{julian2019guaranteeing}. This results in 35 different BNNs which need to be individually verified. Each BNN has one hidden layer with 125 hidden neurons, the same number of hidden neurons studied in the original system \cite{julian2019guaranteeing}.

We use probabilistic local robustness to evaluate whether the network is robust to five properties, referred to as $\phi_0 - \phi_4$ and which correspond to checking the consistency of each possible advisory. These are probabilistic extensions of those considered for NNs in \cite{katz2017reluplex, wang2018formal, julian2019guaranteeing}. For example $\phi_0$ ensures that there is no point inside of the input region which is not classified as COC. In order to perform comprehensive verification of the entire collision avoidance system we discrete the entire input domain into more than 1.8 million different input properties $T$ for which we check the robustness of the ground truth property listed in the dataset and all of the surrounding points. %For each input property, we check that the neural network is probabilistically correct and robust. 
The results of this analysis can be found in the center table of Figure~\ref{fig:HCASTable} \ap{Are you referring to the table or the figure?}. In particular, we find that we are able to certify the probabilistic behavior of all but a very small portion ($> 99\%$) of inputs including guaranteeing correct and robustly correct behavior on more than 77\% of the input space. For another 21\% of the input space, however, we can guarantee that the network is robustly incorrect\ap{Robustly incorrect? To me as an expression it seems to mean that it robustly returns the same incorrect answer. I don't think that is the case. I think you mean that is we guarantee that it can be attacked (as in the upperbound guarantees that). Maybe find a better explanation? E.g. simply incorrect.}. That is to say that for almost all of the functions represented by the BNN the input is certified to be unsafe. A practitioner could further analyze this 21\% to reason about if the system is still safe for deployment \ap{I don't understand this sentence and I don't see why it would need to go here rather than on a discussion on the bound}. This case study and the results obtained validate the value of Algorithm~\ref{alg:simplereachability} \ap{Is not clear to a reader how this statement follows from what you have just said. Rather than stating something like this, try to show it in facts.}.% The benefits of calibrated uncertainty in the case of airborne collision avoidance are clear: if there is a case which is not captured by the training data, we would not like for a confident advisory to be issued. However, calibrated uncertainty is typically not achievable with deterministic neural networks and so one would seek to use Bayesian neural networks. Despite the value of Bayesian neural networks in this setting, it was previously impossible to verify the correctness of their behavior. Thus, it was impossible to deploy BNNs in this setting. Through the guarantees of Algorithm~\ref{alg:simplereachability}, we can now employ Bayesian  neural networks in airborne collision avoidance and a host of other tasks with similar requirements. 

In the bottom row of Figure~\ref{fig:HCASAnalysis}, we study the decision robustness of the system. In order to do so, we take a coarser descritization of the input space resulting in thousands of inputs with width $\epsilon = 0.125$. In the bottom left of Figure~\ref{fig:HCASAnalysis}, we perform a comparative analysis of the certification we can achieve with our method on VI and HMC. We find that in almost all cases we are able to produce a greater certification \ap{What's a greater certification? You mean like a tighter bound, or just a higher bound? As in we observe that the value of the bounds computed for HMC are grater than those computed for VI?} for the discrete HMC posterior over the continuous VI posterior. We hypothesize that this is due to both the improved performance that we expect from HMC posteriors as well as the fact that weight intervals have zero width when certifing HMC which allows for tighter certification.
\ap{This is not super-satisfactory of an explanation. I get it that this is the best you can get out of the current results. But a reviewer might interpret it just as meaning that our bound for VI sucks, which isn't a great thing... It would be good to somehow quantify to what degree the improved bound is affected by HMC vs VI posterior approximation and to what degree is affected by over-approximation due to weight intervals. One way could be to report also upper-bounds (if they are non-vacuous), or to report statistical approximations – and then comments on the gaps.}
We then further study the maximum and minimum posterior predictive softmax values for the VI posterior on $\phi_0$. We find that our method for deriving these bounds is extremely tight \ap{I would drop quantifiers as 'extreme' and similar, because tightness or non-tightness of a bound, i.e., its tollerance, is all relative to the application. 0.1 can be very little (and is ofc impressive given the difficulty of the property), but in something extremely dangerous a 10 percent error can be a lot. Best thing to just drop the quantifiers in this case and report on the tightness observed.}, resulting in a difference that is less that 0.1 on average (seen in the bottom right of Figure~\ref{fig:HCASAnalysis}). This means that for a given decision by the Bayesian posterior, we can guarantee that the posterior predictive mean fall within a tight range which allows us to easily reason about correct behavior.



\subsection{UCI Industrial Regression}

In this section, we study two safety-critical industrial regression problems. Both of these problems have been used before to benchmark approximate Bayesian inference in \cite{hernandez2015probabilistic, gal2016dropout, khan2018fast}. Each datasets has a one dimensional, real-valued output posing a regression problem. Both are taken from \cite{ucidata}. The Concrete dataset involves predicting the compressive strength of concrete based on 8 key factors including its ingredients and age. Failure in this task or overestimation of the compressive strength could lead to the construction of structurally unsound buildings. The Powerplant dataset uses six years worth of observations from combined cycle power plants and poses the problem of predicting energy output from a plant given a range of environmental and plant parameters. Incorrect predictions on this could lead to unsafe settings which could potentially result in failure or underperformance of the plant.

For each dataset, we train a corresponding Bayesian neural network using the Variational Online Gauss Newton (VOGN) method proposed in \cite{khan2018fast}. In particular, we set up their network \ap{You mean the network used in the latter work? I had difficulties parsing this sentence maybe rewrite as "In partiular we rely on the same NN architecture used in the latter work, i.e., a single..." }, a single hidden layer neural network with 100 hidden units and rectified linear unit (ReLU) activation functions. We find that we are able to roughly reproduce the same performance as the authors of \cite{khan2018fast} before turning our attention to the robustness of the resulting posteriors. For each dataset there are several cross-validation splits provided. We provide analysis for Bayesian neural networks trained on the first cross-validation split.

\paragraph{Safe and Unsafe Radius Estimation}

In our analysis of the HCAS dataset we use fixed discretizations of the entire input space \ap{Why do you put this here?}.  One interesting question to ask is: how large can an $\epsilon$-ball be before we can no longer guarantee safety. Similarly, we might ask how small can an $\epsilon$-ball be before we can no longer guarantee unsafety. We call these problems the maximum safe radius (MSR) and minimum unsafe radius (MUR) problems, respectively. These radius values are probabilistic extensions of corresponding deterministic problem which has been studied for deterministic neural networks \cite{wu2018game}. In order to compute this radius we perform a linear search over the values of epsilon. Starting at $\epsilon = 0.01$, if probabilistic robustness is verified to be greater than 0.7 \ap{0.7 is an arbitrary value. If we just put it like this, someone is gonna ask us how we have selected it and why. If insteady we say a given $\lambda$ and then at the end of the explanation we say, we chose this $\lambda$ to be equal to 0.7, though any other reasonable threshold of safety could be used - then it seems more scientific} then we declare the input robust for that radius, increase the $\epsilon$, and recheck. Similarly, for MUR, we start at $\epsilon = 1.0$. If we guarantee that the probabilistic robustness is less than 0.7, then we declare the radius to be unsafe, decrease the value of $\epsilon$, and recheck. The result of these procedures are a sound value for the MSR and MUR respectively. 

We compute both of these values for every test instance on the industrial datasets described and find that we are able to get tight bounds on the true value of MSE and MUR. In the left hand plot of Figure~\ref{fig:UCIAnalysis}, we see that the Concrete dataset is typically guaranteed to be robust up to $0.03$ but is, typically guaranteed to be unsafe past $0.05$. The Powerplant posterior is more robust. We are able to guarantee a MSR of roughly $0.18$ for most inputs, and have that for most inputs the prediction is unsafe for $0.3$. We further analyze our bounds on the MSE and MUR in the center and right hand plots in Figure~\ref{fig:UCIAnalysis}. In each plot we show the per-test-instance MSE and MUR. We find the general and encouraging trend that as MUR increases so does the MSE. 

\subsection{MNIST}

In this section, we turn our attention to a larger dimensionality example than those considered in our prior analyses. MNIST is a well-studied, small-scale image recognition datast. The dataset poses the problem of handwritten digit recognition. Each input is a 28 by 28 (784 dimensional) black and white image which encodes the pen stroke corresponding to a digit 0 through 9. A few examples are given on the far left of Figure~\ref{fig:MNISTAnalysis}.  In order to learn on MNIST we use the standard 50,000/10,000 test/train split that is provided \cite{lecun1998mnist}. For each tested posterior, we again train using the VOGN algorithm from \cite{khan2018fast}. %Our learning rate parameters is chosen based on a randomly selected validation set which is separated from the training set randomly at the beginning of each run. 
In this section, we will study several different architecture configurations; we tune the learning rate parameters for each architecture individually. Each architecture uses rectified linear units as activation functions and a softmax as its final layer. We take the likelihood of the model to be the sparse categorical cross-entropy. 

\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.5\textwidth]{Figures/MNIST_Arch.pdf}}
    \caption{\textbf{Left:} We show the distribution of maximum safe radii and minimum unsafe radii for a BNN with 128 hidden units. \textbf{Right:} For a range of architectures we plot the mean certified safe and unsafe radii. We find that as the network gets deeper the minimum unsafe radius increases. }
    \label{fig:MNISTArch}
\end{figure}

\paragraph{Architecture Complexity} In order to study how the choice of architecture affects the provable robustness of BNNs we vary both the width and depth of a fully connected BNN. We take the safe outputs, $S$, to be the set of softmax vectors such that the true class is maximal (i.e., we ensure that the classification is correct and robust). As we increase the width of the neural network (keeping all else equal, including the parameters of the algorithm) we see a slight decrease in MSR. However, as we increase depth we observe a noticeable increase in the computed MUR. This indicates that increasing the depth of a BNN increases the computational burden of certification more than increasing the width. We hypothesize that this comes from the approximation introduced by convex relaxation techniques.

\paragraph{Correctness and Uncertainty Properties} Unlike the other domains we have studied the space of natural images is extremely large. Thus, predictions on out-of-distribution points become cause for concern. In the center right of Figure~\ref{fig:MNISTAnalysis} we show black and white images of articles of clothing from the FashionMNIST dataset. Of course, they bare no resemblance to the handwritten digits of MNIST, and we should expect a properly calibrated BNN to reflect this with uncertainty in its posterior predictive distribution. In the right hand plot of Figure~\ref{fig:MNISTAnalysis}, we demonstrate how we can use our framework to guarantee robust uncertainty. In order to do so, we take 1000 test set images from the FasionMNIST dataset and we compute upper bounds on the mean of their posterior predictive softmax probability. the information from $\epsilon = 0.05$ we can see that nearly every tested point falls below a critical uncertainty threshold (in this case chosen to be 0.4). What this means is that there is no manipulation of the tested FashionMNIST images which forces our BNN to make an over-confident prediction. Moreover, we can see that this is true up until $\epsilon = 0.07$.

In addition to uncertainty properties, we perform this analysis on the correctness property for a BNN trained on MNIST. In the left hand plot of Figure~\ref{fig:MNISTAnalysis}, we see that we can certify the mean of the posterior predictive softmax to be greater than 0.5 for the correct class for $\epsilon$ up to roughly 0.075. This ensures that there is no adversary which can force a misclassification on these points up to $\epsilon = 0.75$.





\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.48\textwidth]{Figures/GTSRB_Large.pdf}} 
    \caption{We study the performance of a Bayesian convolutional neural network (CNN) on a traffic sign recognition benchmark. In the top row we show that we can verify correctness of test inputs. In the bottom three rows we study the show the guarantees we can derive for the BNN on out-of-distribution inputs including non-sense traffic signs (second row), international traffic signs (third row), and random noise (bottom row). For the tested images we find that we are able to reliably certify the uncertainty of the BNN on such out-of-distribution points.}
    \label{fig:GTSRBAnalysis}
\end{figure}



\subsection{GTSRB}

We study the ability of our method to scale to complex safety-critical tasks with high-dimensional inputs (2,352) and complex architectures. In particular, we study a small CNN architecture on the German Traffic Sign Recognition Benchmark (GTSRB). We study a subset of this dataset considering the 5,000 images that represent the `construction ahead' and `50 Km/H speed limit' signs. This poses a binary classification task on which we train a CNN with two convolutional layers and one hidden layer using VOGN. We find that for this BNN we are able to certify the robust prediction of many test-set inputs which can be seen in Figures~\ref{fig:GTSRBTitleFig} and \ref{fig:GTSRBAnalysis}. Given the highly unpredictable nature of autonomous navigation it is also highly desirable to certify the uncertainty of out-of-distribution points on this task. For this we collect free-use images online representing non-sense traffic signs, traffic signs from the United States, and we generate random noise. These three categories represent images on which our Bayesian CNN ought to be uncertain. Interestingly, we find that for all but one image in this set we are able to certify that the BNN is correctly uncertain with decision, posterior predictive, softmax guaranteed to be no greater than 0.55 for all points in a $\ell_\infty$ ball of radius 2/255.



==> Sections/Introduction_old.tex <==
\section{Introduction}
%
Although Neural Networks (NNs) have recently achieved state-of-the-art performance %, and even outperformed human-level accuracy in several regression and classification tasks
\cite{he2015delving}, 
they are %have been shown to be 
susceptible to several vulnerabilities \cite{biggio2018wild}, with adversarial examples being one of the most prominent among them \cite{IntruigingProperties}.
%As a consequence, since the seminal verification work of \cite{reluplex}, several techniques for the worst-case analysis of NNs were proposed \cite{missing,missing,missing} and argued as a necessity when it comes to the prospect of deploying them in safety-critical scenarios \cite{missing}.
Adversarial examples, inputs which despite being classified correctly \ap{This sentence needs to be re-written. An adversarial example is not an input that gets classified correctly, but an input which is crafted from an input that got classified correctly} can be imperceptibly modified to induce an incorrect prediction, are intuitively related to \emph{uncertainty} \ap{I am not sure of adversarial examples are related to uncertainty mean. I think you meant to write something like, adversarial examples might be captured using uncertainty or something on this line – but it is not clear from the way things are phrased at the moment.} \cite{kendall2017uncertainties, bekasov2018bayesian}. Bayesian Neural Networks (BNNs), i.e. NNs with a probability distribution placed over their weights and biases \cite{neal2012bayesian}, have recently been proposed as a potentially more robust learning paradigm \cite{carbone2020robustness}. %\cite{neal2012bayesian,carbone2020robustness}.
While retaining the advantages intrinsic to deep learning (e.g.\ representation learning), BNNs also enable principled evaluation of model uncertainty, which can be taken into account at prediction time to enable safe decision making.

Bayesian neural networks have been shown to come with many practical benefits for adversarial robustness. In \cite{carbone2020robustness}, it is proven that the exact Bayesian posterior for an overparameterized neural network prevents gradient-based attacks from being effective \ap{Rather than writing exact posterior for over-paramterised weight, I would be a bit more general and say something like "uncer certain limiting conditions on the dataset and capacity of the network etc."}. While gradient-free attacks are marginally more effective \cite{yuan2020gradient}, it remains difficult to attack BNNs. Further, Bayesian uncertainty estimates have been shown to empirically flag adversarial examples in \cite{rawat2017adversarial, smith2018understanding}. However, these approaches only consider pointwise uncertainty estimates, that is, specific to a particular test point.
In contrast, probabilistic safety aims at  computing the uncertainty for compact subspaces of %sets of 
input points, thus taking into account worst-case adversarial perturbations of the input point when considering its neighbourhood.
\ap{I don't think the message you are trying to send is actually coming across here. Trying to be more clear of why is important to do verification of BNNs. You say that they are provably robust to gradient based attacks, and that they are moderately robust even to gradient-free attacks. The logical outcome of this is that there is no reason to verify them? I think you want to be more clear on why this paper is important, worth reading etc...}
\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.5\textwidth]{Figures/GTSRB_TitleFig.pdf}}
    \caption{Through probabilistic verification we can guarantee correct behavior. Left: No adversarial example exists for GTSRB BNN and this 50kmph road sign ($\epsilon = 2/255$). Right: BNN is robustly uncertain on nonsense road sign ($\epsilon = 2/255$). }
    \label{fig:GTSRBTitleFig}
\end{figure}

Many techniques have been proposed  for the evaluation of the robustness of BNNs, including generalisation of NN gradient-based adversarial attacks to BNN posterior distribution \cite{liu2018adv}, statistical verification techniques for adversarial settings \cite{cardelli2019statistical}, as well as pointwise (i.e.\ for a specific test point $x^*$) uncertainty evaluation techniques \cite{rawat2017adversarial, smith2018understanding} \ap{But none of this are good enough cause...}. %\cite{feinman2017detecting,smith2018understanding}.
%However, to the best of our knowledge, methods that formally (i.e., with certified bounds) give guarantees on the behaviour of BNNs against adversarial input perturbations in probabilistic settings are missing.
As well as initial methods for sound verification of BNNs. \ap{Not sure what initial methods mean?}

In this paper we present a framework for 
certifying \emph{probabilistic} and  \emph{decision safety} for BNNs. %This is the first work to provide a systematic treatment of these problems for any posterior representation as well as the first method to provide guarantees for the decision of a Bayesian neural network without modification of the posterior.
Given a BNN, a set $T \subseteq \mathbb{R}^m$ in the input space, and a set $S\subseteq \mathbb{R}^{n_c}$ \ap{m, nc etc. appear here for the first time, you gotta introduce stuff carefully, especially since it is a journal paper. Also you should give some understandinf of what T and S are. Chances are we gonna get a reviewer that hasnt got a deep understadning of adversarial examples.} in the output space, probabilistic safety is defined as the probability that for all $x\in T$ the prediction of the BNN is in $S$. Decision safety requires us to compute the worst case posterior predictive mean of the BNN for a given set in input space $T$. Together, we refer to these two notions simply as \textit{safety} for Bayesian neural networks.
In adversarial settings, the input region $T$ is built around the neighborhood of a given test point $x^*$, while the output region $S$ is defined around the BNN prediction on $x^*$, so that safety translates into computing  whether adversarial perturbations of $x^*$ cause small variations in the BNN output. \ap{This presentation is confusing, because you are trying to deal with two different problems formulation at the same time. Imho, I would first define the problem of probabilistic safety and what you do with the method you develop for one of them you get the other one as well with a few changes or soemthing.}
%Note that probabilistic safety represents a probabilistic variant of the notion of safety commonly used to certify deterministic NNs %against adversarial examples
%\cite{ruan2018reachability}.


Unfortunately, computation of notions of safety for a BNN over a compact set $T$ and for an output region $S$ is not trivial, as it involves computing  the probability that a deterministic NN sampled from the BNN posterior is safe (i.e., all the points in a given set are mapped by the network to a given output set), which is known to be NP-complete %problem already
\cite{katz2017reluplex} \ap{I think you might want to introduce some notation to make this statement more understandable}. 
Nevertheless, we derive a method for the computation of a \emph{certified lower and upper bounds} for safety.
In particular,  we show that the computation of safety for BNNs is equivalent to computing the probability measure, w.r.t.\ BNN posterior, of the set of weights for which the resulting deterministic NN is safe, i.e., robust to adversarial perturbations. \ap{I am not sure this is equivalent, or just the definition itself to be honest.}
We compute a subset of such weights, $\hat{H}$, and build on relaxation techniques from non-convex optimisation to check whether, given a compact set $T$ and a safe output region $S$, all the networks instantiated by weights in $\hat{H}$ are safe.
We provide lower bounds for the case of Interval Bound Propagation (IBP) and Linear Bound Propagation (LBP) \ap{IBP and LBP mentioned here for the first time. What are they? You probably want to explain that they are non-convex relaxation techniques? Also you want to say that we \textit{design} IBP and LBP techniques for BNNs - because we are the first to do so, it's a contribution!} for BNNs trained with Gaussian variational inference (VI) \cite{blundell2015weight} and Hamiltonian Monte Carlo (HMC) methods. However, we note that the derived bounds can be extended to other approximate Bayesian inference techniques. %\ap{Mention somewhere that we do experiments just for VI but the bound is general.}

We experimentally investigate the behaviour of our method on the airborne collision avoidance system (ACAS), industrial regression datasets from the UCI dataset repository, and the MNIST image recognition dataset. % for a range of properties and different BNN architectures, and applying bounds obtained both via IBP and LBP.
We show that our method allows one to compute non-trivial, certified lower bounds on the probabilistic safety of BNNs with millions of weights in a few minutes. \ap{You got to give something more interesting here.} %hundreds of seconds.
%We provide comparison between bounds obtained via IBP and via LBP and discuss relative merits and cases in which one method is preferable to the other. 





%Bayesian models have recently attracted great interest for application in safety-critical scenarios because of their ability to capture uncertainty, which could be propagated through the decision pipeline in order to enable safe decision making \cite{mcallister2017concrete,michelmore2019uncertainty}. In particular,
%Bayesian Neural Networks (BNNs), i.e.,  neural networks with a distribution over their weights, retain  the main   advantages   intrinsic   to   deep   neural   networks while also enabling principled characterization of the uncertainty in the learning model \cite{neal2012bayesian}.
%However, methods that formally (i.e., with certified bounds)  give guarantees on the behavior of a BNN against adversarial perturbations, while also accounting for its stochastic nature, are missing with existing methods that are either limited to statistical approaches \cite{cardelli2019statistical} or only consider pointwise robustness measures of uncertainty \cite{feinman2017detecting,smith2018understanding}. 

%In this paper we want to evaluate  \emph{probabilistic safety} for a BNN. Given a BNN, a set in the input space $T \subseteq \mathbb{R}^m$, and a set in the output space $S\subseteq \mathbb{R}^{n_c}$, probabilistic safety is defined as the probability that for all $x\in T$ the prediction of the BNN are in $S$. 
%Note that probabilistic safety represents a probabilistic generalization of the notion of safety  commonly used to certify deterministic neural networks against  adversarial examples \cite{ruan2018reachability}. %Moreover,
%it is a measure widely employed to guarantee the safety of  models exhibiting a probabilistic behaviour \cite{abate2008probabilistic} and .
%For instance, probabilistic safety can be used to quantify the safety of a model learned with a BNN in a model-based reinforcement learning scenario or to formally compute the uncertainty of the BNN predictions in a decision problem setting.
%\LL{Here, we could given some examples of why it is  cool. (A sketch is commented in there)}
 %and their computation allows one to also compute the satisfaction probability of more general properties \cite{}. \LL{This second part of the sentence may be not needed}. 
 


%Unfortunately, the computation of probabilistic safety for BNNs is far from being trivial, as it requires to compute the probability that a deterministic neural network sampled from the BNN posterior is safe (i.e., all of the test points of a given set are mapped from the network in a given output set). 
%Hence, we develop a method for the computation of a \emph{certified lower bound} of probabilistic safety.
%In particular,  we show that the computation of probabilistic safety for BNNs is equivalent to compute the set of weights for which the resulting deterministic neural network is safe and  we derive a framework for the computing of a lower bound of such a set. 


In summary, this paper makes the following main contributions.\footnote{An implementation to reproduce all the experiments can be found at: \url{https://github.com/matthewwicker/ProbabilisticSafetyforBNNs}.  }

\begin{itemize}
    \item  We propose %derive 
    a framework based on relaxation techniques from non-convex optimisation
    for the %safe 
    %computation of the 
    analysis of 
    probabilistic and decision safety for BNNs with general \ap{General is a bit of an over-statement, go for commonly used.} activation functions and multiple hidden layers.
    %\item We derive techniques for computing the set of weights such that the BNN is safe for each of this weight, employing Interval Bound Propagation (IBP) or Linear Bound Propagation (LBP). \LL{Improve this one}  
    \item We derive explicit procedures based on IBP and LBP for the computation of the set of weights for which the corresponding NN sampled from the BNN posterior distribution is safe.
    \item We establish methods for computing sound bounds on the posterior probability of sets of weights for any posterior representation. \ap{Not sure what this sentence mean.}
    \item  On various datasets we show that our algorithm \ap{you mean method?} can efficiently verify multi-layer BNNs with millions of parameters in a few minutes.
\end{itemize}
\ap{From the contribution you miss the fact that you get provable bounds! You also probably want to explicitly state in the introduction that a preliminary version of this paper was published at blah blah blah. And this paper improves it in a number of different way. The main ones being: blah blah blah}

\section{Related Work}

Most existing certification methods %for the  of neural networks 
are designed for deterministic neural networks (see e.g., \cite{katz2017reluplex}) and cannot be used for verification of Bayesian models against probabilistic properties. In particular, in \cite{weng2018towards,zhang2018efficient,gowal2018effectiveness}  Interval Bound Propagation (IBP) and Linear Bound Propagation (LBP) approaches have been employed for certification of deterministic neural networks. 
%We also note the existence of other methods of certification such as abstract interpretation \cite{gehr2018ai2} and linear programming \cite{tjeng2017evaluating}.
However, these methods cannot be used for BNNs because they all assume that the weights of the networks are deterministic, i.e\ fixed to a given value, while in the Bayesian setting we need to certify the BNN for a continuous range of values for weights that are not fixed, but distributed according to the BNN posterior.
We extend IBP and LBP to BNNs in Section \ref{subsec:convexrelax}. %and show how they can be used to compute probabilistic safety.




%gradient-based attacks for BNNs have been developed in \cite{liu2018adv}. However, these methods are empirical and cannot guarantee the existence or absence of adversarial points.
A probabilistic property analogous to one considered in this paper has been studied for BNNs in \cite{cardelli2019statistical, michelmore2019uncertainty}.
However, the solution methods presented in \cite{cardelli2019statistical, michelmore2019uncertainty} are statistical, with confidence bounds, and in practice cannot give certified guarantees for the computed values, which are important for safety-critical applications.
Our approach, instead building on non-linear optimisation relaxation techniques, computes a certified lower bound.

%Formal
Methods to compute probabilistic adversarial measures of robustness in Bayesian learning settings have been explored for Gaussian Processes (GPs),  both for regression \cite{cardelli2018robustness} and classification tasks \cite{grosse2018limitations, blaas2019robustness, wicker2021bayesian}.
However, the vast majority of inference methods employed for BNNs do not have a Gaussian approximate distribution in latent/function space, even if they assume a Guassian distribution in the weight space \cite{blundell2015weight}.
Hence, certification techniques for GPs cannot be directly employed for BNNs. 
%This also includes BNNs trained with variational inference, where a Gaussian distribution is assumed in the weight space (e.g., Bayes by Backprop \cite{blundell2015weight}).
In fact, because of the non-linearity of the BNN structure, even in this case the distribution of the BNN is not Gaussian in function space. 
Though methods to approximate BNN inference with GP-based inference have been proposed \cite{emtiyaz2019approximate}, the guarantees obtained in this way would apply to the approximation and not the actual BNN, and would not provide error bounds. 
In contrast, our method is specifically tailored to take into account the non-linear nature of BNNs and can be directly applied to a range of approximate Bayesian inference techniques.

Finally there are a few works which study certified robustness guarantees for Bayesian neural networks. In [UAI2021] the authors extend the notion of probabilistic robustness for Bayesian neural networks to finite-horizon iterative prediction problems. Here, we cover a more diverse range of properties for single prediction tasks as well as decision robustness. In \cite{berrada2021make} the authors truncate mean-field Gaussian posteriors in order to soundly reason about predictive quantities from BNNs. In this work, we do not modify the posterior in any way and can deal with a variety of posterior representations. In addition, we scale to larger BNNs. \ap{This things need to get discussed together with when you discuss BNNs verificaiton above (or all down here).}



  
  





==> Sections/Limitations.tex <==
\section{Limitations}
\ap{Note to my self: Embed this partially int he conclusion, partially in the experiments, partially in the methods, and get rid of this section}
In this Section, we highlight four key limitations of our methods and results which may be taken as future work. Here we specifically discuss weaknesses in the properties we can explore, the lack convergence of our bounds to the true value, the adverse affect of posterior variance, as well as the lack of ability to scale to complex modern architectures.

In our experiments, we highlight the various ways in which our bounds on probabilistic and decision robustness can aid practitioners in analysis of adversarial behavior of their BNNs. However, each of these applications models the input set $T$ as an $\ell_\infty$-norm ball. While this is the most widely used robustness measure and captures a subset of the properties of interest, it cannot be readily adapted to more complex semantic properties. While our framework can handle sets $T$ which are defined as convex polytopes, these may also be insufficient for pertinent safety specifications. Other works have moved towards certifying such sophisticated semantic perturbations \cite{mohapatra2020towards}, but more work needs to be done to adapt these to the BNN setting. It is clear that these properties can be adapted to finite-time horizon properties such as reach-avoid specifications \cite{wicker2021certification}, but we do not explore this setting in this work.



A final practical limitation of our method is the inability of this method to readily scale to complex, modern neural architectures. In image classification it is common to use networks with over 50 sequential hidden layers. However, the conservative nature of bound propagation means that our method can only handle networks that are less than 10 hidden layers deep. Moreover, sequential prediction tasks often use more complicated mechanisms such as GRUs \cite{chung2014empirical} and LSTMs \cite{hochreiter1997long} which we do not study in this work. Certification of such architectures is important for wide spread use of certification techniques and is an important area of future research.


